Timed Runtime Monitoring for Multiparty Conversations

We propose a dynamic verification framework for protocols in real-time distributed systems. The framework is based on Scribble, a tool-chain for design and verification of choreographies based on multiparty session types, developed with our industrial partners. Drawing from recent work on multiparty session types for real-time interactions, we extend Scribble with clocks, resets, and clock predicates constraining the times in which interactions should occur. We present a timed API for Python to program distributed implementations of Scribble specifications. A dynamic verification framework ensures the safe execution of applications written with our timed API: we have implemented dedicated runtime monitors that check that each interaction occurs at a correct timing with respect to the corresponding Scribble specification. The performance of our implementation and its practicability are analysed via benchmarking.

==> eptcsdata.tex <==
\providecommand{\firstpage}{19}
\providecommand{\publicationstatus}{Marco Carbone (Ed.): Third Workshop on\\
Behavioural Types (BEAT 2014)\\
EPTCS 162, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.162.3}{10.4204/EPTCS.162.3}}
\pdfoutput=1

